Knapsack on Graphs with Relaxed Neighborhood Constraints

In the knapsack problems with neighborhood constraints that were studied before, the input is a graph $\mathcal{G}$ on a set $\mathcal{V}$ of items, each item $v \in \mathcal{V}$ has a weight $w_v$ and profit $p_v$, the size $s$ of the knapsack, and the demand $d$. The goal is to compute if there exists a feasible solution whose total weight is at most $s$ and total profit is at most $d$. Here, feasible solutions are all subsets $\mathcal{S}$ of the items such that, for every item in $\mathcal{S}$, at least one of its neighbors in $\mathcal{G}$ is also in $\mathcal{S}$ for \hor, and all its neighbors in $\mathcal{G}$ are also in $\mathcal{S}$ for \hand~\cite{borradaile2012knapsack}. We study a relaxation of the above problems. Specifically, we allow all possible subsets of items to be feasible solutions. However, only those items for which we pick at least one or all of its neighbor (out-neighbor for directed graph) contribute to profit whereas every item picked contribute to the weight; we call the corresponding problems \sor and \sand. We show that both \sor and \sand are strongly \NPC even on undirected graphs. Regarding parameterized complexity, we show both \sor and \hor are \WTH parameterized by the size $s$ of the knapsack size. Interestingly, both \sand and \hand are \WOH parameterized by knapsack size, $s$ plus profit demand, $d$ and also parameterized by solution size, $b$. For \sor and \hor, we present a randomized color-coding-based pseudo-\FPT algorithm, parameterized by the solution size $b$, and consequently by the demand $d$. We then consider the treewidth of the input graph as our parameter and design pseudo fixed-parameter tractable (\FPT) algorithm parameterized by treewidth, $\text{tw}$ for all variants. Finally, we present an additive $1$ approximation for \sor when both the weight and profit of every vertex is $1$.

==> approximation.tex <==
\section{Approximation Algorithms}
In this section we discuss the feasibility of polynomial time approximation algorithms.

\subsection{Given a target profit $d$, minimize cost or weight}
\begin{definition}[\sor]
    Given a directed graph $\GG = (\VV, \EE)$, where each vertex $u \in \VV$ has a weight $w_u$ and a profit $p_u$, a knapsack of size $s$, and a demand $d$, compute a subset $\VV^\prime \subseteq \VV$ such that:
    \begin{enumerate}
        %\item if $u \in \VV^\prime$, then at least one of its out-neighbors must also be in $\VV^\prime$.
        \item $\forall u \in \VV^\prime$, if any of its out-neighbors is not selected (i.e., $u \in \VV^\prime$ for some $(u, v) \in \EE$, such that $v \not \in \VV^\pr$), then include $w_u$ in the total weight, but do not include $p_u$ in the total profit.
        \item Let $\VV^{\pr\pr} \subseteq \VV^\pr$ be the set of vertices such that at least one of its out-neighbors is not selected in $\VV^\pr$.
        \item $\sum_{u \in \VV^\pr} w_u \leq s$.
        \item $\sum_{u \in \VV^\pr \setminus \VV^{\pr\pr}} p_u \geq d$.
    \end{enumerate}
\end{definition}
\begin{align*}
    \text{minimize} \quad & \sum_{u \in \VV} w_u x_u  \\
    \text{subject to} \quad & \sum_{u \in \VV} p_u z_u \geq d, \\
    & z_u \leq x_u, \quad \forall u \in \VV, \\
    & z_u \leq \sum_{v: (u,v) \in \EE}x_v, \quad \forall u \in \VV, \\
    & x_u, z_u \in \{0, 1\}, \quad \forall u \in \VV.
\end{align*}

\textcolor{red}{What about vertices with 0 out degree? This ILP does not capture that}

\begin{observation}
    The relaxed LP of the above ILP has bad integrality gap.
\end{observation}

\begin{align*}
    \text{minimize} \quad & \sum_{u \in \VV} w_u x_u  \\
    \text{subject to} \quad & \sum_{u \in \VV \setminus \UU} p_u^{\UU} z_u \geq d_{\UU}, \quad \forall \UU \subseteq \VV \\
    & z_u \leq x_u, \quad \forall u \in \VV, \\
    & z_u \leq \sum_{v: (u,v) \in \EE}x_v, \quad \forall u \in \VV, \\
    & x_u, z_u \in \{0, 1\}, \quad \forall u \in \VV.
\end{align*}

\textcolor{red}{What about vertices with 0 out degree? This ILP does not capture that}

\begin{definition}[\sand]
    Given a directed graph $\GG = (\VV, \EE)$, where each vertex $u \in \VV$ has a weight $w_u$ and a profit $p_u$, a knapsack of size $s$, and a demand $d$, compute a subset $\VV^\prime \subseteq \VV$ such that:
    \begin{enumerate}
        %\item if $u \in \VV^\prime$, then at least one of its out-neighbors must also be in $\VV^\prime$.
        \item $\forall u \in \VV^\prime$, if all its out-neighbors are not selected (i.e., $u \in \VV^\prime$ for some $(u, v) \in \EE$  such that $v \not \in \VV^\pr$), then include $w_u$ in the total weight, but do not include $p_u$ in the total profit.
         \item Let $\VV^{\pr\pr} \subseteq \VV^\pr$ be the set of vertices such that all of its out-neighbors are not selected in $\VV^\pr$.
        \item $\sum_{u \in \VV^\prime} w_u \leq s$.
        \item $\sum_{u \in \VV^\pr \setminus \VV^{\pr\pr}} p_u \geq d$.
    \end{enumerate}
\end{definition}
\begin{align*}
    \text{minimize} \quad & \sum_{u \in \VV} w_u x_u  \\
    \text{subject to} \quad & \sum_{u \in \VV} p_u z_u \geq d, \\
    & z_u \leq x_u, \quad \forall u \in \VV, \\
    & z_u \leq x_v, \quad \forall(u,v) \in \EE, \\
    & x_u, z_u \in \{0, 1\}, \quad \forall u \in \VV.
\end{align*}


\begin{observation}
    The relaxed LP of the above ILP has bad integrality gap.
\end{observation}

\begin{align*}
    \text{minimize} \quad & \sum_{u \in \VV} w_u x_u  \\
    \text{subject to} \quad & \sum_{u \in \VV \setminus \UU} p_u^{\UU} z_u \geq d_{\UU}, \quad \forall \UU \subseteq \VV \\
    & z_u \leq x_u, \quad \forall u \in \VV, \\
    & z_u \leq x_v, \quad \forall(u,v) \in \EE, \\
    & x_u, z_u \in \{0, 1\}, \quad \forall u \in \VV.
\end{align*}

\subsection{Given a knapsack of size $s$, maximize profit}

\textcolor{red}{The result below was observed in Hard version reference: \cite{borradaile2012knapsack}}.
\begin{observation}\label{sor-apx-hard}
  \sor has no \((1 - \frac{1}{e} + \epsilon)\)-factor approximation algorithm for any $\epsilon > 0$ unless \Pb = \NP.
\end{observation}
\begin{proof}
    Consider an instance of ([n], $\{S_i\}_{i = 1}^m$, $k$, $t$) of \mc problem.  We construct an instance of \sor as follows:
\begin{enumerate}
    \item Consider a bipartite graph $\GG(\VV=\AA\cup\BB,\EE)$ with the bi-partition as follows
    \begin{itemize}
        \item Let \AA be the set of [n] elements of the universe.
        \item Let \BB be the set of [m] sets of the universe.
    \end{itemize}
    \item Define \(\EE = \{\{i,j\} : j \in \AA \text{ and } i \in \BB \text{ and } j \in S_i \text{ for } i \in [m]\}\)
    \item Assign the weights as 
        \[w_u =
            \begin{cases}
                0 & \text{if } u \in \AA, \\
                1 & \text{if } u \in \mathcal{B}.
            \end{cases}
         \]
    \item Assign the profits as 
        \[p_u =
            \begin{cases}
                1 & \text{if } u \in \AA, \\
                0 & \text{if } u \in \mathcal{B}.
            \end{cases}
         \]
    \item Set $s = k$ and $d = t$
\end{enumerate}
This is exactly the \mc problem and the reduction is approximation preserving. 
\end{proof}

\begin{corollary}\label{sor-apx-hard-gen}
  \sor has no \((1 - \frac{1}{e} + \epsilon)\)-factor approximation algorithm for any $\epsilon > 0$ unless \Pb = \NP for maximizing profit in directed graphs and general graphs.
\end{corollary}

\begin{observation}\label{sand-apx-hard}
  \sand has no \(\OO (n^{(1 - \epsilon)})\)-factor approximation algorithm for any $\epsilon > 0$ unless \Pb = \NP for maximizing profit in bipartite graphs.
\end{observation}
\begin{proof}
    Given an instance of \clique as $(\GG^\pr = (\VV^\pr, \EE^\pr), k)$, we construct an instance of \sand as follows:
\begin{enumerate}
    \item Consider a bipartite graph $\GG(\VV=\AA\cup\BB,\EE)$ with the bi-partition as follows
    \begin{itemize}
        \item Let \AA be the set of vertices in $\GG^\pr$.
        \item Let \BB be the set of edges in $\GG^\pr$. Thus, each vertex $v \in \BB$ has degree exactly 2, since each $e \in \EE^\pr$ is incident on 2 vertices.
    \end{itemize}
    \item Define \(\EE = \{ \{e, u\}, \{e, v\} \mid e \in \BB, \text{ and } u, v \in \AA, \forall e = (u, v) \in \EE^\pr \} \)
    \item Assign the weights as 
        \[w_u =
            \begin{cases}
                1 & \text{if } u \in \AA, \\
                0 & \text{if } u \in \BB.
            \end{cases}
         \]
    \item Assign the profits as 
        \[p_u =
            \begin{cases}
                0 & \text{if } u \in \AA, \\
                1 & \text{if } u \in \BB.
            \end{cases}
         \]
    \item Set $s = k$ and $d = \binom{k}{2}$
\end{enumerate}
This is exactly the \clique problem and the reduction is approximation preserving. We know that \clique cannot be approximated within \( n^{(1 - \epsilon)} \).
\end{proof}

\begin{corollary}\label{sand-apx-hard-gen}
  \sand has no \(\OO (n^{(1 - \epsilon)})\)-factor approximation algorithm for any $\epsilon > 0$ unless \Pb = \NP for maximizing profit in directed graphs and general graphs.
\end{corollary}

==> color_coding_vertices.tex <==
\begin{theorem}
    There exists a randomized color coding based $\OO\left(e^b\cdot b^b\cdot 2^{b^2}\cdot n^{\OO(1)}\cdot {\sf min}\{s^2,p^2\}\right)$ pseudo-\FPT algorithm for \sor parameterized by solution size (budget) $b$.
\end{theorem}

\begin{proof}    
  We color the vertices of the given graph, with the hope that each vertex in our desired optimal solution gets distinctly colored. The solution is a subset of vertices and selected vertices induce a forest in \GG where each component is of size at least 2. \textcolor{red}{discuss why solution looks like this} We color the instance so that the desired structure (if exists) gets highlighted with decent probability. \textcolor{red}{We aim to partition the colors into subsets, where each subset corresponds to a tree in the solution. }
  
  Color the vertices uniformly at random from $\{1,2,\dots,b\}$ and guess $k$ partitions of [b]: $\CC_1, \CC_2, \CC_3, \dots, \CC_k$ such that each partition is a tree of size at least 2 and no two partitions have the same color class i.e. let the set of colors in $\CC_i$ be denoted by $\chi(\CC_i)$, then $\chi(\CC_i)$ $\cap$ $\chi(\CC_j)$ = $\emptyset$, $\forall i, j \in [k]$ where $i \neq j$. We iterate over all possible choices of $k$. Note that $1 \leq k \leq \frac{b}{2}$.\textcolor{red}{For the rest of the algorithm we assume that we have rightly guessed such partitions with distinct colors.}

 % Consider a partition $\CC_i$. Let $\tau(\CC_i)$ denote the set of all trees in $\CC_i$. We design a dynamic programming based algorithm to find a tree with maximum profit such that each vertex in this tree is distinctly colored and the profit is maximized across this partition.

 Consider a partition $\CC_i$. Let $\tau(\CC_i)$ denote the set of all trees in $\CC_i$. We design a dynamic programming based algorithm to find a colorful tree with the exact structure and if this is the case, then the algorithm returns all feasible and undominated pairs of the colorful tree. There may be multiple witness of such a tree however we maintain only undominated pairs. %\textcolor{red}{in $\CC_i$ we are finding a colorful tree of size ???? with that exact structure.}

  \textbf{Dynamic Programming} We apply dynamic programming: for a non empty tree $T(X)$ and a vertex $u \in \bigcup_{i \in [k]}\CC_i$, we define the state $D[T(\XX),u]$ to store a list of all the feasible undominated weight and profit pairs i.e ${(w,p)}$ corresponding to \XX-colorful tree $T(\XX) \in \tau(\CC_i)$ having vertex $u$.

D[T(X),u] should store all undominated feasible weight-profit pairs for a colorful tree T(X) that uses each color in X exactly once, contains u as a vertex, and has a structure dictated by the tree T(X). Since each color appears exactly once in T(X), there is a unique choice for  vertex $u$ corresponding to that color. 

To compute the DP state \( D[T(X), u] \), which stores all undominated feasible weight-profit pairs for a colorful tree \( T(X) \) rooted at vertex \( u \), we observe that each color in \( X \) appears exactly once in \( T(X) \), meaning the vertex \( u \) is uniquely determined by its color. A sanity check condition ensures that if the color of \( u \), \( \chi(u) \), does not belong to \( T(X) \), then \( D[T(X), u] = \emptyset \), as no valid tree structure can exist.

For the base case where \( |X| = 1 \), the tree \( T(X) \) consists of a single vertex \( u \). We define:

\[
D[T(X), u] =
\begin{cases} 
\{(w_u, p_u)\}, & \text{if } \chi(u) \in X, \\
\emptyset, & \text{otherwise}.
\end{cases}
\]

For the base case where \( |X| = 2 \), \( T(X) \) is a single edge \( \{u, v\} \), and we define:

\[
D[T(X), u] =
\begin{cases} 
\{(w_u + w_v, p_u + p_v)\}, & \text{if } \chi(u), \chi(v) \in X \text{ and } (u,v) \in E(G), \\
\emptyset, & \text{otherwise}.
\end{cases}
\] 

For \( |X| \geq 3 \), we construct \( D[T(X), u] \) by cutting an edge in the tree \( T(X) \). Specifically, we identify an edge in \( T(X) \) connecting two colors, \( c_1 \) and \( c_2 \), where \( c_1 = \chi(u) \) is the unique color of \( u \) in \( T(X) \). The color \( c_2 \) must belong to a neighbor of \( u \) in \( T(X) \); otherwise, no valid tree structure can exist. We partition the color set into two disjoint subsets \( X' \) and \( X \setminus X' \), such that \( c_1 \in X \setminus X' \) and \( c_2 \in X' \), and decompose \( T(X) \) into two subtrees:  
1. \( T(X \setminus X') \), which remains rooted at \( u \).  
2. \( T(X') \), which must be rooted at a vertex \( v \) that has color \( c_2 \) and is a neighbor of \( u \) in \( G \).  

Since multiple vertices in \( G \) can have color \( c_2 \), we iterate over all such feasible neighbors \( v \) where \( (u, v) \in E(G) \) and combine the DP values:
\[
D[T(X), u] = D[T(X \setminus X'), u] \oplus D[T(X'), v]
\]
where \( \oplus \) merges weight-profit pairs while maintaining only undominated pairs. This transition ensures that the structure of \( T(X) \) is respected and that the DP state efficiently aggregates the best possible combinations. Finally we save only the undominated pairs. \textcolor{red}{write this properly. currently this is not so clear...}

We repeat the algorithm across all partitions to ensure all possible trees are considered, yielding the final output. Now we add the weight and profit from each of these partitions $\CC_1, \CC_2, \CC_3, \dots, \CC_k$ and output \(\max \{ p \mid (w, p) \text{ is a feasible pair and } w \leq s \}\). \textcolor{red}{change runtime to $\min\{s,d\}^2\cdot (k-1)$}

We now show that the algorithm runs in time $\OO\left(e^b\cdot b^b\cdot 2^{b^2}\cdot n^{\OO(1)}\cdot {\sf min}\{s^b,p^b\}\right)$, and given a \yes instance, returns a solution with probability at least $e^{-b}$. By repeating the algorithm independently, $e^{b}$ times, we obtain the running time bound. The color coding technique assigns \( b \) colors uniformly at random to all vertices in the graph. The probability that a fixed solution of size \( b \) gets assigned distinct colors is at least \( e^{-b} \). To boost this probability to a constant (e.g., at least \( 1/2 \)), we repeat the random coloring \( e^b \) times. For each coloring, we iterate over all possible ways to partition the \( b \) colors into disjoint subsets, where each subset corresponds to a tree of size at least 2. The number of such partitions is upper bounded by \( b^b \). For each color subset (i.e., tree), we guess a rooted tree structure over those colors, and the number of possible rooted trees over at most \( b \) colors is bounded by \( 2^{b^2} \). For each such tree structure, we perform dynamic programming over all vertices in the graph to compute all undominated feasible \((w,p)\) pairs. The number of such pairs is bounded by \( \min\{s^b, p^b\} \), since we only store undominated combinations under the budget constraint \( w \leq s \) and demand requirement \( p \geq d \). Each DP computation involves traversing the tree and combining child subtrees, which can be done in polynomial time per vertex. Therefore, the overall running time is $\OO\left(e^b\cdot b^b\cdot 2^{b^2}\cdot n^{\OO(1)}\cdot {\sf min}\{s^b,p^b\}\right)$
as claimed.

\end{proof}

